Towards Knowledge-Based Recommender Dialog System

In this paper, we propose a novel end-to-end framework called KBRD, which stands for Knowledge-Based Recommender Dialog System. It integrates the recommender system and the dialog generation system. The dialog system can enhance the performance of the recommendation system by introducing knowledge-grounded information about users' preferences, and the recommender system can improve that of the dialog generation system by providing recommendation-aware vocabulary bias. Experimental results demonstrate that our proposed model has significant advantages over the baselines in both the evaluation of dialog generation and recommendation. A series of analyses show that the two systems can bring mutual benefits to each other, and the introduced knowledge contributes to both their performances.

==> 2-problem.tex <==
\section{Problem Formulation}
% requires more details

TODO

\paragraph{\it Definition 1} \textbf{Multi-turn conversation}
$C = (q_{1:T}, a_{1:T}) = (q_1, a_1, q_2, a_2, \ldots, q_T, a_T)$. $q_t$, $a_t$ each represents a sentence.
\dm{$C = \{(q_1, a_1),\ldots, (q_T,a_T)\}$}
% \paragraph{\it Definition 2} \textbf{Movies} mentioned in a conversation: $M = (m_1, \ldots, m_K)$, $m_k$ an entity.

% \paragraph{\it Definition 3} \textbf{User feedback} on mentioned movies $M$: $S = (s_1, \ldots, s_k)$. $s_i \in \left\{Like, Dislike, Unk\right\}$.

\paragraph{Task} At conversation turn $t < T$, with conversation history $q_{1:t}, a_{1:t-1}$ and movies mentioned $m_{1:l-1}$, generate a natural response $a_t$, can be asking for the user's interest or recommending a movie $m_l$ (optional).
\dm{Problem should be defined more detailed. How many dialogues for a user? Any other information?}
